M2L Translation Operators for Kernel Independent Fast Multipole Methods on Modern Architectures

Hardware trends favor algorithm designs that maximize data reuse per FLOP. We develop and benchmark high-performance Multipole-to-Local (M2L) translation operators for the kernel-independent Fast Multipole Method (kiFMM), a widely adopted FMM variant that supports a broad class of kernels and has been favored by recent implementations for its simple specification. Naively implemented, M2L is bandwidth-limited and therefore a key bottleneck in the FMM. State-of-the-art FFT-based M2L implementations, though elegant and with a fast setup time, suffer from low operational intensity and require architecture-specific optimizations. We demonstrate that a BLAS-based M2L, combined with randomized low-rank compression, achieves competitive performance with greater portability and a simpler implementation leveraging existing BLAS infrastructure, at the cost of higher setup times-especially for high-accuracy settings in double precision. Our Rust-based implementation enables seamless switching between strategies for fair benchmarking. Results on CPUs show that FFT-based M2L is favorable in low-accuracy settings or dynamic particle simulations, while BLAS-based M2L is favored for high-accuracy settings for static particle distributions, where its higher setup costs are amortized in many practical applications of the FMM.

==> Makefile <==
TEXFILE=draft
LATEX=pdflatex
BIB=bibtex
GLOSS=makeglossaries

.PHONY: all clean $(TEXFILE).pdf

all: $(TEXFILE).pdf

$(TEXFILE).pdf:
	$(LATEX) $(TEXFILE).tex; \
	${BIB} $(TEXFILE); \
	$(LATEX) $(TEXFILE).tex; \
	$(LATEX) $(TEXFILE).tex; \

clean:
	rm -f *.aux *.log *.bbl *.blg *.glg *.glo *.gls *.ist *.acn *.acr *.alg \
	      *.out *.toc *.lof *.lot *.fls *.fdb_latexmk *.run.xml *.xdy *.synctex.gz *.glsdefs $(TEXFILE).pdf


==> images/laplace_singular_values_error_single.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-1.25, xmax=26.25,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\(\displaystyle \epsilon\)},
ymin=-0.79529730107736, ymax=2.27372131829548,
ytick style={color=black},
xlabel style={scale=2}, % Scaling the x-axis label
ylabel style={scale=2}, % Scaling the x-axis label
tick label style={scale=2} % This line sets the tick label size
]
\addplot [semithick, steelblue31119180]
table {%
0 0
1 -0.115302804831248
2 -0.115322832539247
3 -0.115330703234353
4 -0.307950574667744
5 -0.307968212702041
6 -0.307993272341266
7 -0.0711286926061714
8 -0.0711356183280234
9 -0.547232120417541
10 -0.301734931477585
11 -0.301752977291097
12 -0.301808229377354
13 -0.225846603638037
14 -0.225863555713728
15 -0.225885419853234
16 -0.655796454742231
17 -0.526748476109117
18 -0.526789999311023
19 -0.526799341281795
20 -0.247594916376757
21 -0.247628216230726
22 0.450444582001506
23 0.374237593814906
24 0.374221286311488
25 0.556163457675989
};
\draw (axis cs:3,1.8) node[
  scale=2,
  text=black,
  rotate=0.0
]{$p=3$};

\nextgroupplot[
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-4.85, xmax=101.85,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.79529730107736, ymax=2.27372131829548,
ytick style={color=black},
yticklabels={},
xlabel style={scale=2}, % Scaling the x-axis label
tick label style={scale=2} % This line sets the tick label size
]
\addplot [semithick, steelblue31119180]
table {%
0 0
1 -0.0288102829159418
2 -0.0288290704493304
3 -0.0288363257447393
4 -0.0842538863635989
5 -0.0842684567788661
6 -0.0842899878333458
7 -0.027917607360104
8 -0.0279240062176136
9 -0.163442986685029
10 -0.101779274455393
11 -0.10179436424565
12 -0.101848096537279
13 -0.0838453959735164
14 -0.0838581147084048
15 -0.0838794953461077
16 -0.221102632039311
17 -0.18652128684632
18 -0.186554352536151
19 -0.186557285131804
20 -0.0568940368878081
21 -0.0569172949866834
22 -0.0329870189950423
23 -0.109207432774187
24 -0.109229856321577
25 -0.20239077066732
26 -0.202493838683719
27 -0.202589326824735
28 -0.131387096487913
29 -0.131389482806004
30 -0.198259473176602
31 -0.198317866833905
32 -0.198357609563515
33 -0.045849652666659
34 -0.0459171312978928
35 -0.0459514839236785
36 -0.291501336643947
37 -0.291565069999539
38 -0.291777419936295
39 -0.236121630718268
40 -0.179825244132894
41 -0.179859806736376
42 -0.249095792750547
43 -0.219863570495137
44 -0.122653231619358
45 -0.122665987283582
46 -0.162901373609623
47 0.151685681619401
48 -0.0260192213946446
49 0.228953255372854
50 -0.0144222711985584
51 -0.0145643267782649
52 -0.0149183408893929
53 -0.185564911820753
54 -0.186459076602238
55 -0.186701144057515
56 -0.150579754950654
57 -0.150704637397457
58 -0.0683639076342022
59 -0.0689886463777949
60 -0.0694446730457532
61 0.0110079757290382
62 0.010745644578396
63 0.0106398994780079
64 -0.0767364553138528
65 -0.0780001232512237
66 -0.0780766702036697
67 -0.33542196550998
68 -0.0967897034365013
69 -0.0970006503265388
70 -0.262296373536074
71 -0.264107784166702
72 -0.265213555342022
73 0.0912373485941735
74 0.0913291084658141
75 0.10443746957732
76 0.0152717454373512
77 0.0152207061750822
78 -0.0116830830878865
79 -0.0164279086788515
80 -0.0188103889860862
81 0.275703450498456
82 0.574252393107791
83 0.729847344901264
84 0.374278505044753
85 0.372874706575846
86 0.316951308107893
87 0.32354219628338
88 0.318942402170698
89 0.582158106262254
90 0.85355058860223
91 0.85078008607586
92 1.2776415842213
93 1.1822663159048
94 1.44150581410022
95 1.84446911632687
96 1.7894373101866
97 2.13422047196035
};
\draw (axis cs:-5,1.8) node[
  scale=2,
  anchor=west,
  text=black,
  rotate=0.0
]{$p=5$};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!1.2!(current bounding box.north west)$}) node[
  scale=2,
  anchor=north,
  text=black,
  rotate=0.0
]{Single Precision};

\end{tikzpicture}


==> images/rcmp_double_precision.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
    height=8cm,
    width=15cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Rank \(\displaystyle k\)},
xmin=-2.14, xmax=58.14,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Frequency},
ymin=0, ymax=180.6,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:0.6,0) rectangle (axis cs:0.866666666666667,172);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180}
\addlegendentry{$\epsilon = 10^{-4}$}

\draw[draw=none,fill=steelblue31119180] (axis cs:1.6,0) rectangle (axis cs:1.86666666666667,48);
\draw[draw=none,fill=steelblue31119180] (axis cs:2.6,0) rectangle (axis cs:2.86666666666667,42);
\draw[draw=none,fill=steelblue31119180] (axis cs:3.6,0) rectangle (axis cs:3.86666666666667,54);
\draw[draw=none,fill=steelblue31119180] (axis cs:4.6,0) rectangle (axis cs:4.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:5.6,0) rectangle (axis cs:5.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:6.6,0) rectangle (axis cs:6.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:7.6,0) rectangle (axis cs:7.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:8.6,0) rectangle (axis cs:8.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:9.6,0) rectangle (axis cs:9.86666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:10.6,0) rectangle (axis cs:10.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:11.6,0) rectangle (axis cs:11.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:12.6,0) rectangle (axis cs:12.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:13.6,0) rectangle (axis cs:13.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:14.6,0) rectangle (axis cs:14.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:15.6,0) rectangle (axis cs:15.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:16.6,0) rectangle (axis cs:16.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:17.6,0) rectangle (axis cs:17.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:18.6,0) rectangle (axis cs:18.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:19.6,0) rectangle (axis cs:19.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:20.6,0) rectangle (axis cs:20.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:21.6,0) rectangle (axis cs:21.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:22.6,0) rectangle (axis cs:22.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:23.6,0) rectangle (axis cs:23.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:24.6,0) rectangle (axis cs:24.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:25.6,0) rectangle (axis cs:25.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:26.6,0) rectangle (axis cs:26.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:27.6,0) rectangle (axis cs:27.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:28.6,0) rectangle (axis cs:28.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:29.6,0) rectangle (axis cs:29.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:30.6,0) rectangle (axis cs:30.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:31.6,0) rectangle (axis cs:31.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:32.6,0) rectangle (axis cs:32.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:33.6,0) rectangle (axis cs:33.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:34.6,0) rectangle (axis cs:34.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:35.6,0) rectangle (axis cs:35.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:36.6,0) rectangle (axis cs:36.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:37.6,0) rectangle (axis cs:37.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:38.6,0) rectangle (axis cs:38.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:39.6,0) rectangle (axis cs:39.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:40.6,0) rectangle (axis cs:40.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:41.6,0) rectangle (axis cs:41.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:42.6,0) rectangle (axis cs:42.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:43.6,0) rectangle (axis cs:43.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:44.6,0) rectangle (axis cs:44.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:45.6,0) rectangle (axis cs:45.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:46.6,0) rectangle (axis cs:46.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:47.6,0) rectangle (axis cs:47.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:48.6,0) rectangle (axis cs:48.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:49.6,0) rectangle (axis cs:49.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:50.6,0) rectangle (axis cs:50.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:51.6,0) rectangle (axis cs:51.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:52.6,0) rectangle (axis cs:52.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:53.6,0) rectangle (axis cs:53.8666666666667,0);
\draw[draw=none,fill=steelblue31119180] (axis cs:54.6,0) rectangle (axis cs:54.8666666666667,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:0.866666666666667,0) rectangle (axis cs:1.13333333333333,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714}
\addlegendentry{$\epsilon = 10^{-7}$}

\draw[draw=none,fill=darkorange25512714] (axis cs:1.86666666666667,0) rectangle (axis cs:2.13333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:2.86666666666667,0) rectangle (axis cs:3.13333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:3.86666666666667,0) rectangle (axis cs:4.13333333333333,32);
\draw[draw=none,fill=darkorange25512714] (axis cs:4.86666666666667,0) rectangle (axis cs:5.13333333333333,36);
\draw[draw=none,fill=darkorange25512714] (axis cs:5.86666666666667,0) rectangle (axis cs:6.13333333333333,24);
\draw[draw=none,fill=darkorange25512714] (axis cs:6.86666666666667,0) rectangle (axis cs:7.13333333333333,72);
\draw[draw=none,fill=darkorange25512714] (axis cs:7.86666666666667,0) rectangle (axis cs:8.13333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:8.86666666666667,0) rectangle (axis cs:9.13333333333333,98);
\draw[draw=none,fill=darkorange25512714] (axis cs:9.86666666666667,0) rectangle (axis cs:10.1333333333333,24);
\draw[draw=none,fill=darkorange25512714] (axis cs:10.8666666666667,0) rectangle (axis cs:11.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:11.8666666666667,0) rectangle (axis cs:12.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:12.8666666666667,0) rectangle (axis cs:13.1333333333333,24);
\draw[draw=none,fill=darkorange25512714] (axis cs:13.8666666666667,0) rectangle (axis cs:14.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:14.8666666666667,0) rectangle (axis cs:15.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:15.8666666666667,0) rectangle (axis cs:16.1333333333333,6);
\draw[draw=none,fill=darkorange25512714] (axis cs:16.8666666666667,0) rectangle (axis cs:17.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:17.8666666666667,0) rectangle (axis cs:18.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:18.8666666666667,0) rectangle (axis cs:19.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:19.8666666666667,0) rectangle (axis cs:20.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:20.8666666666667,0) rectangle (axis cs:21.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:21.8666666666667,0) rectangle (axis cs:22.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:22.8666666666667,0) rectangle (axis cs:23.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:23.8666666666667,0) rectangle (axis cs:24.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:24.8666666666667,0) rectangle (axis cs:25.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:25.8666666666667,0) rectangle (axis cs:26.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:26.8666666666667,0) rectangle (axis cs:27.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:27.8666666666667,0) rectangle (axis cs:28.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:28.8666666666667,0) rectangle (axis cs:29.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:29.8666666666667,0) rectangle (axis cs:30.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:30.8666666666667,0) rectangle (axis cs:31.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:31.8666666666667,0) rectangle (axis cs:32.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:32.8666666666667,0) rectangle (axis cs:33.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:33.8666666666667,0) rectangle (axis cs:34.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:34.8666666666667,0) rectangle (axis cs:35.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:35.8666666666667,0) rectangle (axis cs:36.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:36.8666666666667,0) rectangle (axis cs:37.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:37.8666666666667,0) rectangle (axis cs:38.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:38.8666666666667,0) rectangle (axis cs:39.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:39.8666666666667,0) rectangle (axis cs:40.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:40.8666666666667,0) rectangle (axis cs:41.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:41.8666666666667,0) rectangle (axis cs:42.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:42.8666666666667,0) rectangle (axis cs:43.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:43.8666666666667,0) rectangle (axis cs:44.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:44.8666666666667,0) rectangle (axis cs:45.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:45.8666666666667,0) rectangle (axis cs:46.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:46.8666666666667,0) rectangle (axis cs:47.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:47.8666666666667,0) rectangle (axis cs:48.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:48.8666666666667,0) rectangle (axis cs:49.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:49.8666666666667,0) rectangle (axis cs:50.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:50.8666666666667,0) rectangle (axis cs:51.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:51.8666666666667,0) rectangle (axis cs:52.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:52.8666666666667,0) rectangle (axis cs:53.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:53.8666666666667,0) rectangle (axis cs:54.1333333333333,0);
\draw[draw=none,fill=darkorange25512714] (axis cs:54.8666666666667,0) rectangle (axis cs:55.1333333333333,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:1.13333333333333,0) rectangle (axis cs:1.4,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=forestgreen4416044}
\addlegendentry{$\epsilon = 10^{-10}$}

\draw[draw=none,fill=forestgreen4416044] (axis cs:2.13333333333333,0) rectangle (axis cs:2.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:3.13333333333333,0) rectangle (axis cs:3.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:4.13333333333333,0) rectangle (axis cs:4.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:5.13333333333333,0) rectangle (axis cs:5.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:6.13333333333333,0) rectangle (axis cs:6.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:7.13333333333333,0) rectangle (axis cs:7.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:8.13333333333333,0) rectangle (axis cs:8.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:9.13333333333333,0) rectangle (axis cs:9.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:10.1333333333333,0) rectangle (axis cs:10.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:11.1333333333333,0) rectangle (axis cs:11.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:12.1333333333333,0) rectangle (axis cs:12.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:13.1333333333333,0) rectangle (axis cs:13.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:14.1333333333333,0) rectangle (axis cs:14.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:15.1333333333333,0) rectangle (axis cs:15.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:16.1333333333333,0) rectangle (axis cs:16.4,92);
\draw[draw=none,fill=forestgreen4416044] (axis cs:17.1333333333333,0) rectangle (axis cs:17.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:18.1333333333333,0) rectangle (axis cs:18.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:19.1333333333333,0) rectangle (axis cs:19.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:20.1333333333333,0) rectangle (axis cs:20.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:21.1333333333333,0) rectangle (axis cs:21.4,48);
\draw[draw=none,fill=forestgreen4416044] (axis cs:22.1333333333333,0) rectangle (axis cs:22.4,24);
\draw[draw=none,fill=forestgreen4416044] (axis cs:23.1333333333333,0) rectangle (axis cs:23.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:24.1333333333333,0) rectangle (axis cs:24.4,8);
\draw[draw=none,fill=forestgreen4416044] (axis cs:25.1333333333333,0) rectangle (axis cs:25.4,78);
\draw[draw=none,fill=forestgreen4416044] (axis cs:26.1333333333333,0) rectangle (axis cs:26.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:27.1333333333333,0) rectangle (axis cs:27.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:28.1333333333333,0) rectangle (axis cs:28.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:29.1333333333333,0) rectangle (axis cs:29.4,12);
\draw[draw=none,fill=forestgreen4416044] (axis cs:30.1333333333333,0) rectangle (axis cs:30.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:31.1333333333333,0) rectangle (axis cs:31.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:32.1333333333333,0) rectangle (axis cs:32.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:33.1333333333333,0) rectangle (axis cs:33.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:34.1333333333333,0) rectangle (axis cs:34.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:35.1333333333333,0) rectangle (axis cs:35.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:36.1333333333333,0) rectangle (axis cs:36.4,24);
\draw[draw=none,fill=forestgreen4416044] (axis cs:37.1333333333333,0) rectangle (axis cs:37.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:38.1333333333333,0) rectangle (axis cs:38.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:39.1333333333333,0) rectangle (axis cs:39.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:40.1333333333333,0) rectangle (axis cs:40.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:41.1333333333333,0) rectangle (axis cs:41.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:42.1333333333333,0) rectangle (axis cs:42.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:43.1333333333333,0) rectangle (axis cs:43.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:44.1333333333333,0) rectangle (axis cs:44.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:45.1333333333333,0) rectangle (axis cs:45.4,24);
\draw[draw=none,fill=forestgreen4416044] (axis cs:46.1333333333333,0) rectangle (axis cs:46.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:47.1333333333333,0) rectangle (axis cs:47.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:48.1333333333333,0) rectangle (axis cs:48.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:49.1333333333333,0) rectangle (axis cs:49.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:50.1333333333333,0) rectangle (axis cs:50.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:51.1333333333333,0) rectangle (axis cs:51.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:52.1333333333333,0) rectangle (axis cs:52.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:53.1333333333333,0) rectangle (axis cs:53.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:54.1333333333333,0) rectangle (axis cs:54.4,0);
\draw[draw=none,fill=forestgreen4416044] (axis cs:55.1333333333333,0) rectangle (axis cs:55.4,6);
\end{axis}

\end{tikzpicture}

